Leading the Pack: N-player Opponent Shaping

Reinforcement learning solutions have great success in the 2-player general sum setting. In this setting, the paradigm of Opponent Shaping (OS), in which agents account for the learning of their co-players, has led to agents which are able to avoid collectively bad outcomes, whilst also maximizing their reward. These methods have currently been limited to 2-player game. However, the real world involves interactions with many more agents, with interactions on both local and global scales. In this paper, we extend Opponent Shaping (OS) methods to environments involving multiple co-players and multiple shaping agents. We evaluate on over 4 different environments, varying the number of players from 3 to 5, and demonstrate that model-based OS methods converge to equilibrium with better global welfare than naive learning. However, we find that when playing with a large number of co-players, OS methods' relative performance reduces, suggesting that in the limit OS methods may not perform well. Finally, we explore scenarios where more than one OS method is present, noticing that within games requiring a majority of cooperating agents, OS methods converge to outcomes with poor global welfare.

==> global_welfare.tex <==

\begin{table}
    \centering
    \caption{Converged Global Welfare by different methods on Staghunt, Tragedy of the commons (ToC), Snowdrift and the Iterated Prisoners Dilemma (IPD). Here we see how across all environments \textsc{SHAPER} outperforms LOLA. Secondly we note that across Staghunt and Snowdrift games, OS methods fail to produce better results than the Naive baseline. Results are reported over N seeds with mean and standard deviation.}
    \label{tab:my-table}
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{Method} & \textbf{Staghunt 3} & \textbf{Staghunt 4} & \textbf{Staghunt 5} & \textbf{ToC 3} & \textbf{ToC 4} & \textbf{ToC 5} \\
        \midrule
        \textbf{Naive} & 0.00 ± 0.00 & 0.00 ± 0.00 & 0.00 ± 0.00 & 0.00 ± 0.00 & 0.00 ± 0.00 & 0.00 ± 0.00 \\
        \textbf{LOLA} & 0.40 ± 0.38 & 0.04 ± 0.16 & -0.04 ± 0.06 & 1.03 ± 0.66 & -0.33 ± 0.90 & -0.11 ± 0.51 \\
        \textbf{Shaper} & 3.00 ± 1.48 & 0.37 ± 0.06 & 0.04 ± 0.00 & 4.98 ± 0.00 & 0.41 ± 0.78 & 3.93 ± 0.87 \\
        \midrule
        \textbf{Method} & \textbf{Snowdrift 3} & \textbf{Snowdrift 4} & \textbf{Snowdrift 5} & \textbf{IPD 3} & \textbf{IPD 4} & \textbf{IPD 5} \\
        \midrule
        \textbf{Naive} & 2.05 ± 0.68 & 2.52 ± 0.14 & 3.77 ± 0.05 & 1.00 ± 0.00 & 1.00 ± 0.01 & 3.42 ± 0.09 \\
        \textbf{LOLA} & 1.95 ± 0.43 & 2.72 ± 0.30 & 3.68 ± 0.42 & 1.33 ± 0.29 & 2.27 ± 0.55 & 3.37 ± 0.31 \\
        \textbf{Shaper} & 2.99 ± 0.00 & 3.15 ± 0.71 & 3.60 ± 0.03 & 4.80 ± 0.10 & 4.18 ± 1.23 & 4.96 ± 0.79 \\
        \bottomrule
    \end{tabular}
\end{table}


==> os_welfare.tex <==


\begin{table}
    \centering
    \caption{Naive baseline and opponent shaper welfare of players LOLA and 1 Shaper}
    \label{tab:my-table}
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{Method} & \textbf{Staghunt 3} & \textbf{Staghunt 4} & \textbf{Staghunt 5} & \textbf{ToC 3} & \textbf{ToC 4} & \textbf{ToC 5} \\
        \midrule
        \textbf{Naive} & 0.00 ± 0.00 & 0.00 ± 0.00 & 0.00 ± 0.00 & 0.00 ± 0.00 & 0.00 ± 0.00 & 0.00 ± 0.00 \\
        \textbf{LOLA} & 0.40 ± 0.38 & '0.04 ± 0.16' & '-0.04 ± 0.06' & '1.03 ± 0.66' & '-0.33 ± 0.90' & '-0.11 ± 0.51' \\
        \textbf{1 Shaper} & 3.00 ± 1.48 & '0.37 ± 0.06' & '0.04 ± 0.00' & '4.98 ± 0.00' & '0.41 ± 0.78' & '3.93 ± 0.87' \\
        \midrule
        \textbf{Method} & \textbf{Snowdrift 3} & \textbf{Snowdrift 4} & \textbf{Snowdrift 5} & \textbf{IPD 3} & \textbf{IPD 4} & \textbf{IPD 5} \\
        \midrule
        \textbf{Naive} & 2.05 ± 0.68 & 2.52 ± 0.14 & 3.77 ± 0.05 & 1.00 ± 0.00 & 1.00 ± 0.01 & 3.42 ± 0.09 \\
        \textbf{LOLA} & 1.95 ± 0.43 & '2.72 ± 0.30' & '3.68 ± 0.42' & '1.33 ± 0.29' & '2.27 ± 0.55' & '3.37 ± 0.31' \\
        \textbf{1 Shaper} & 2.99 ± 0.00 & '3.15 ± 0.71' & '3.60 ± 0.03' & '4.80 ± 0.10' & '4.18 ± 1.23' & '4.96 ± 0.79' \\
        \bottomrule
    \end{tabular}
\end{table}



==> results_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\centering
\begin{tabular}{lllllll}
\hline

\multicolumn{1}{|l|}{{\ul \textit{\textbf{Staghunt}}}} &
  \multicolumn{1}{l|}{\textbf{naive}} &
  \multicolumn{1}{l|}{\textbf{LOLA}} &
  \multicolumn{1}{l|}{\textbf{1 SHAPER}} &
  \multicolumn{1}{l|}{\textbf{2 SHAPER}} &
  \multicolumn{1}{l|}{\textbf{3 SHAPER}} &
  \multicolumn{1}{l|}{\textbf{4 SHAPER}} \\ \hline
  
\multicolumn{1}{|l|}{\textbf{3pl}} &
  \multicolumn{1}{c|}{0.00 ± 0.00} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.62 ± 0.77\\  0.40 ± 0.38 \\ 0.73 ± 0.88\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}1.71 ± 1.45\\\red{3.00 ± 1.48} \\ \blue{1.07 ± 0.91}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{2.00 ± 1.41}\\ 2.50 ± 1.50\\ \blue{1.00 ± 0.01}\end{tabular}} &
  \multicolumn{1}{c|}{X} &
  \multicolumn{1}{c|}{X} \\ \hline
  
\multicolumn{1}{|l|}{\textbf{4pl}} &
  \multicolumn{1}{c|}{0.00 ± 0.00} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{0.14 ± 0.44}\\  0.04± 0.16 \\ \blue{0.18 ± 0.50}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}-0.08 ± 0.27\\  \red{0.37 ± 0.06}\\ -0.23 ± 0.10\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.00 ± 0.00\\ 0.00 ± 0.00\\ 0.00 ± 0.00\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.00 ± 0.00\\ 0.00 ± 0.00\\ 0.00 ± 0.00\end{tabular}} &
  \multicolumn{1}{c|}{X} \\ \hline
  
\multicolumn{1}{|l|}{\textbf{5pl}} &
  \multicolumn{1}{l|}{0.00 ± 0.00} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.00 ± 0.04\\ -0.04 ± 0.06 \\  0.01 ± 0.03\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}-0.29 ± 0.16\\ \red{0.04 ± 0.00}\\ -0.4 ± 0.02\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.00 ± 0.00\\ 0.00 ± 0.00\\ 0.00 ± 0.00\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.00 ± 0.00\\ 0.00 ± 0.00\\ 0.00 ± 0.00\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.00 ± 0.00\\ 0.00 ± 0.00\\ 0.00 ± 0.00\end{tabular}} \\ \hline



 &
   &
   &
   &
   &
   &
   \\ \hline





   
\multicolumn{1}{|l|}{{\ul \textit{\textbf{ToC}}}} &
  \multicolumn{1}{l|}{\textbf{naive}} &
  \multicolumn{1}{l|}{\textbf{LOLA}} &
  \multicolumn{1}{l|}{\textbf{1 SHAPER}} &
  \multicolumn{1}{l|}{\textbf{2 SHAPER}} &
  \multicolumn{1}{l|}{\textbf{3 SHAPER}} &
  \multicolumn{1}{l|}{\textbf{4 SHAPER}} \\ \hline
\multicolumn{1}{|l|}{\textbf{3pl}} &
  \multicolumn{1}{c|}{0.00 ± 0.00} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1.35 ± 1.23\\ 1.03 ± 0.66\\ 1.51 ± 1.40\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{2.99 ± 1.41}\\ \red{4.98 ± 0.00}\\ \blue{1.99 ± 0.00}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{2.99 ± 1.41}\\ 3.50 ± 1.41\\ \blue{2.00 ± 0.00}\end{tabular}} &
  \multicolumn{1}{c|}{X} &
  \multicolumn{1}{c|}{X} \\ \hline
  
\multicolumn{1}{|l|}{\textbf{4pl}} &
  \multicolumn{1}{c|}{0.00 ± 0.00} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-0.08 ± 0.47\\ -0.33 ± 0.90\\  0.00 ± 0.01\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{0.33 ± 1.33}\\ \red{0.41 ± 0.78}\\ \blue{0.30 ± 1.47}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.00 ± 0.00\\ 0.00 ± 0.00\\ 0.00 ± 0.00\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.00 ± 0.00\\ 0.00 ± 0.00\\ 0.00 ± 0.00\end{tabular}} &
  \multicolumn{1}{c|}{X} \\ \hline
  
\multicolumn{1}{|l|}{\textbf{5pl}} &
  \multicolumn{1}{l|}{0.00 ± 0.00} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.10 ± 0.35\\ -0.11 ± 0.51\\  0.15 ± 0.27\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{2.47 ± 0.99}\\ \red{3.93 ± 0.87}\\ \blue{2.11 ± 0.62}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.00 ± 0.00\\ 0.00 ± 0.00\\ 0.00 ± 0.00\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.00 ± 0.00\\ 0.00 ± 0.00\\ 0.00 ± 0.00\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.00 ± 0.00\\ 0.00 ± 0.00\\ 0.00 ± 0.00\end{tabular}} \\ \hline
 &
   &
   &
   &
   &
   &
   \\ \hline


   
\multicolumn{1}{|l|}{{\ul \textit{\textbf{Snowdrift}}}} &
  \multicolumn{1}{l|}{\textbf{naive}} &
  \multicolumn{1}{l|}{\textbf{LOLA}} &
  \multicolumn{1}{l|}{\textbf{1 SHAPER}} &
  \multicolumn{1}{l|}{\textbf{2 SHAPER}} &
  \multicolumn{1}{l|}{\textbf{3 SHAPER}} &
  \multicolumn{1}{l|}{\textbf{4 SHAPER}} \\ \hline
\multicolumn{1}{|l|}{\textbf{3pl}} &
  \multicolumn{1}{c|}{2.05 ± 0.68} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}2.10 ± 0.43\\ 1.95 ± 0.43\\  \blue{2.18 ± 0.41}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{2.33 ± 0.58}\\ \red{2.99 ± 0.00}\\ 2.00 ± 0.42\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{2.33 ± 0.94}\\ \red{3.00 ± 0.00}\\ 1.00 ± 0.00\end{tabular}} &
  \multicolumn{1}{c|}{X} &
  \multicolumn{1}{c|}{X} \\ \hline
  
\multicolumn{1}{|l|}{\textbf{4pl}} &
  \multicolumn{1}{c|}{2.52 ± 0.14} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}2.75 ± 0.41\\ 2.72 ± 0.30\\ \blue{2.76 ± 0.44}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}2.56 ± 1.03\\ 3.15 ± 0.71\\ 2.36 ± 1.05\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{3.24 ± 0.80}\\ \red{4.00 ± 0.00}\\ 2.50 ± 0.38\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{3.25 ± 1.30}\\ \red{4.00 ± 0.00}\\ 1.00 ± 0.00\end{tabular}} &
  \multicolumn{1}{c|}{X} \\ \hline
  
\multicolumn{1}{|l|}{\textbf{5pl}} &
  \multicolumn{1}{l|}{3.77 ± 0.05} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}3.81 ± 0.41\\ 3.68 ± 0.42 \\ \blue{3.84 ± 0.41}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}3.02 ± 0.29\\ 3.60 ± 0.03\\ 2.88 ± 0.05\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}2.80 ± 0.46\\ 3.33 ± 0.11\\ 2.44 ± 0.15\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{4.20 ± 1.24}\\ \red{5.00 ± 0.01}\\ 3.00 ± 1.20\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{4.20 ± 1.60}\\ \red{5.00 ± 0.00}\\ 1.00 ± 0.00\end{tabular}} \\ \hline
 &
   &
   &
   &
   &
   &
   \\ \hline


\multicolumn{1}{|l|}{{\ul \textit{\textbf{IPD}}}} &
  \multicolumn{1}{l|}{\textbf{naive}} &
  \multicolumn{1}{l|}{\textbf{LOLA}} &
  \multicolumn{1}{l|}{\textbf{1 SHAPER}} &
  \multicolumn{1}{l|}{\textbf{2 SHAPER}} &
  \multicolumn{1}{l|}{\textbf{3 SHAPER}} &
  \multicolumn{1}{l|}{\textbf{4 SHAPER}} \\ \hline
\multicolumn{1}{|l|}{\textbf{3pl}} &
  \multicolumn{1}{c|}{1.00 ± 0.00} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1.76 ± 0.79 \\ 1.33 ± 0.29\\ 1.99 ± 0.87\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{3.16 ± 1.16}\\ \red{4.80 ± 0.10}\\ \blue{2.35 ± 0.16}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}2.16 ± 1.30\\ 3.07 ± 0.22\\ 0.33 ± 0.12\end{tabular}} &
  \multicolumn{1}{c|}{X} &
  \multicolumn{1}{c|}{X} \\ \hline

  
\multicolumn{1}{|l|}{\textbf{4pl}} &
  \multicolumn{1}{c|}{1.00 ± 0.01} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}2.50 ± 0.94 \\ 2.27 ± 0.55\\ 2.58 ± 1.02\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{4.04 ± 0.70}\\ 4.18 ± 1.23\\ \blue{4.00 ± 0.37}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{4.08 ± 1.30}\\ \red{5.22 ± 0.61}\\ 2.92 ± 0.58\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}2.62 ± 1.38\\ 3.29 ± 0.73\\ 0.60 ± 0.80\end{tabular}} &
  \multicolumn{1}{c|}{X} \\ \hline

  
\multicolumn{1}{|l|}{\textbf{5pl}} &
  \multicolumn{1}{l|}{3.42 ± 0.09} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}3.47 ± 0.97\\ 3.37 ± 0.31\\ 3.50 ± 1.08\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}5.03 ± 0.62\\ 4.96 ± 0.79\\ \blue{5.05 ± 0.57}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{5.43 ± 1.34}\\ \red{7.07 ± 0.25}\\ 4.96 ± 0.79\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}4.31 ± 1.43\\ 5.36 ± 0.58\\ 2.75 ± 0.71\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}2.57 ± 1.16\\ 3.15 ± 0.17\\ 0.26 ± 0.04\end{tabular}} \\ \hline



\end{tabular}
\caption{Converged equilibria across games after 1000 evaluation steps, number of players and opponent shaping agents. Means and standard deviations are reported over 10 seeds for the baseline methods and 5 seeds for SHAPER settings. In each cell the first row corresponds to global welfare, the second to the opponent-shapers' average score, and the third to the naive learners' average score. When all agents are naive learners, we only indicate global welfare. \textbf{Bold}, \blue{blue} and \red{red} indicates the highest \textbf{global}, \red{opponent shaper} and \blue{naive learner} welfare. Xs represent invalid configurations.}
\label{tab:results}
\end{table}
